SEA++: Multi-Graph-based High-Order Sensor Alignment for Multivariate Time-Series Unsupervised Domain Adaptation

Unsupervised Domain Adaptation (UDA) methods have been successful in reducing label dependency by minimizing the domain discrepancy between a labeled source domain and an unlabeled target domain. However, these methods face challenges when dealing with Multivariate Time-Series (MTS) data. MTS data typically consist of multiple sensors, each with its own unique distribution. This characteristic makes it hard to adapt existing UDA methods, which mainly focus on aligning global features while overlooking the distribution discrepancies at the sensor level, to reduce domain discrepancies for MTS data. To address this issue, a practical domain adaptation scenario is formulated as Multivariate Time-Series Unsupervised Domain Adaptation (MTS-UDA). In this paper, we propose SEnsor Alignment (SEA) for MTS-UDA, aiming to reduce domain discrepancy at both the local and global sensor levels. At the local sensor level, we design endo-feature alignment, which aligns sensor features and their correlations across domains. To reduce domain discrepancy at the global sensor level, we design exo-feature alignment that enforces restrictions on global sensor features. We further extend SEA to SEA++ by enhancing the endo-feature alignment. Particularly, we incorporate multi-graph-based high-order alignment for both sensor features and their correlations. Extensive empirical results have demonstrated the state-of-the-art performance of our SEA and SEA++ on public MTS datasets for MTS-UDA.

==> scratch.tex <==




% To cope with such applications, we thus formulate a more challenging yet practical scenario of Multivariate Time-Series Unsupervised Domain Adaptation (MTS-UDA). 


% First, the signals of MTS data originate from multiple sensors where data from different sensors follow various data distributions due to diverse positions of sensors \cite{shi2022deep}. However, current TS UDA methods generally assume that the data from various sensors originate from identical distributions and thus simply treat all sensors as a whole \cite{Cai_Chen_Li_Chen_Zhang_Ye_Li_Yang_Zhang_2021,https://doi.org/10.48550/arxiv.2203.08321}. This scheme may not take the diverse distributions of different sensors into account, against the multi-source nature of MTS data and thus leading to the misalignment of each sensor and sub-optimal solutions of domain adaptation. 




% against the multi-source nature of MTS data. By treating all sensors as a whole, existing UDA methods can consider the global distributions of sensors \cite{https://doi.org/10.48550/arxiv.2203.08321}. But they cannot take the sensor-level distributions into account, leading to the misalignment of each sensor. As presented in Fig.~\ref{fig:SEAnece} (\textbf{Left}), previous UDA methods only align the global features between domains, resulting in the poor alignment of the features from the red sensor and limiting the transferability of the models. 


% This is because the signals in such applications originate from multiple sensors where data from different sensors follow various data distributions due to diverse positions of sensors \cite{shi2022deep}. However, current TS UDA methods generally assume that data originate from one single source \cite{Cai_Chen_Li_Chen_Zhang_Ye_Li_Yang_Zhang_2021} and the various sensors follow identical distributions, against the multi-source nature of MTS data. To cope with such applications, we thus formulate a more challenging yet practical scenario of Multivariate Time-Series Unsupervised Domain Adaptation (MTS-UDA).

% While substantial progress has been made, existing TS UDA methods generally assume that data originate from one single source \cite{Cai_Chen_Li_Chen_Zhang_Ye_Li_Yang_Zhang_2021}. Yet, they are inapplicable for real-world applications where multiple sensors are deployed simultaneously, e.g. remaining useful life (RUL) prediction and human activity recognition (HAR). To cope with such applications, we thus formulate a more challenging yet practical scenario of Multivariate Time-Series Unsupervised Domain Adaptation (MTS-UDA). MTS data originate from multiple sensors where data from different sensors follow various data distributions \cite{}. 


% By treating all sensors as a whole, existing UDA methods can consider the global distributions of sensors \cite{https://doi.org/10.48550/arxiv.2203.08321}. But they cannot take the sensor-level distributions into account, leading to the misalignment of each sensor. As presented in Fig.~\ref{fig:SEAnece} (\textbf{Left}), previous UDA methods only align the global features between domains, resulting in the poor alignment of the features from the red sensor and limiting the transferability of the models. 


% First, the alignment method of SEA at the sensor level is realized with one-order statistics, which is too naive to achieve comprehensive alignment across domains. For example, in SEA, sensor correlations are aligned with the average correlations across domains. Second, SEA ignores the dynamically changing distributions within MTS data. For example, with the degradation of a machine, the status of the machine is changing, so the distributions of sensors would also dynamically change. The ignorance of the information would restrict the performance of domain adaptation.

\section{related work}


% Additionally, some adversarial-based works \cite{wang2020self} have been designed to consider the diverse effects of individual samples.

% Li et al. \cite{li2019domain} argued the importance of task-specific features, so designed association reinforcement to align the features.






% aligning the sensor features between domains. We assume that the features from the same sensor should show similar distributions. 
% Meanwhile, compared with features from the same sensors, features from different sensors between domains should have distinct properties. 
% For example, as shown in Fig. \ref{fig:corralign} \textbf{Middle}, the distribution of sensor 1 in the source domain should be more similar to the distribution of the corresponding sensor in the target domain than to the distributions of other sensors (e.g., sensors 2, 3, and 4) in the target domain.
% To achieve this goal, we propose a sensor contrasting mechanism that facilitates the alignment of sensor features between domains.


% Similar to SCA, the sensor contrasting mechanism is realized with the training batches in source and target domains. Given training batches with $n^s$ and $n^t$ samples in source and target domains, we define the sensor features of the $T$-th graph as $\mathcal{Z}_T^s\in\mathbb{R}^{n^s\times{N}\times{d}}$ and $\mathcal{Z}_T^t\in\mathbb{R}^{n^t\times{N}\times{d}}$ in source and target domains respectively. Here, $\mathcal{Z}_T^s = \{\mathcal{Z}_{n,T}^s\}_{n=1}^N$, where $\mathcal{Z}_{n,T}^s = \{z^s_{i,n,T}\}_{i}^{n^s}$.
% In SFA, the contrasting between domains was performed using the averaged sensor features. As shown in Eq. (\ref{eq:SFA}), here $z_{n,T}^s = \sum_i^{n^s}z^s_{i,n,T}/n^s$ is the averaged sensor features over a training batch.
% % In particular, SFA obtained the average features in domains, e.g., the features of sensor $n$ are obtained by $p_{n,T}^s = \sum_i^{n^s}z^s_{i,n,T}/n^s$ and then the contrasting is achieved by Eq. (\ref{eq:SFA}). 
% \begin{equation}
%     \label{eq:SFA}
%     \begin{split}
%         \mathcal{L}_{SFA,T} &= -\frac{1}{N}\sum_n^Nlog\frac{e^{\varphi(z_{m,T}^s, z_{m,T}^t)}}{\sum_{z_{j,T}^t\in{P^t}}e^{\varphi(z_{m,T}^s, z_{j,T}^t)}},\\
%         &\varphi(z_{m,T}^s, z_{m,T}^t) = z_{m,T}^s(z_{m,T}^{t})^T.
%     \end{split}
% \end{equation}
% SFA encounters a similar challenge as SCA. Specifically, the alignment procedure described in Eq. (\ref{eq:SFA}) relies on first-order statistics and may not fully capture the variance present within complex distributions. To overcome this limitation, we enhance SFA and introduce a new method called iSFA (improved SFA), which incorporates Deep Coral into the contrasting process.

% In Eq. (\ref{eq:iSFA}), iSFA begins by calculating the sensor-level distribution discrepancy using Deep Coral, which takes into account second-order statistics. Subsequently, iSFA leverages the discrepancies to perform contrasting between domains, i.e., minimizing the distribution discrepancy between the same sensors across domains while maximizing the distribution discrepancy between different sensors across domains. This approach allows for more comprehensive alignment of sensor features.
% \begin{equation}
%     \label{eq:iSFA}
%     \begin{split}
%         \mathcal{L}_{iSFA,T} = -\frac{1}{N}\sum_n^Nlog\frac{e^{M_c(\mathcal{Z}_{n,T}^s,\mathcal{Z}_{n,T}^t})}{\sum^N_{j}e^{M_c(\mathcal{Z}_{n,T}^s,\mathcal{Z}_{j,T}^t)}}.
%     \end{split}
% \end{equation}
%         % \\
%         % \varphi(p_m^s, p_m^t) &= p_m^s(p_m^{t})^T.
% % where $L^t = \{l_m^t\}_{m=1}^N$.
% \paragraph{Multi-Graph Alignment}
% To combine the sensor feature alignment and sensor correlation alignment in each sequential graph, a naive approach would be to directly average them.
% However, the distributions between domains at different graphs might show various discrepancies. To account for this and achieve better domain adaptation, we propose learning weights for adjustment, as shown in Eq. (\ref{eq:multi_align}).
% \begin{equation}
%     \label{eq:multi_align}
%     \begin{split}
%         \mathcal{L}_{Endo} &= \sum_T\mathcal{W}_T(\lambda_{SCA}\mathcal{L}_{iSCA,T}+\lambda_{SFA}\mathcal{L}_{iSFA,T}),\\
%         \mathcal{W}_T &= M_c([\mathcal{Z}_{1,T}^s,...,\mathcal{Z}_{\hat{L},T}^s],[\mathcal{Z}_{1,T}^t,...,\mathcal{Z}_{\hat{L},T}^t]),
%     \end{split}
% \end{equation}
% where $[a,...,b]$ represents concatenating the elements from $a$ to $b$. Eq. (\ref{eq:multi_align}) represents that the learnable weights $\mathcal{W}_T$ are obtained by computing the distribution discrepancy of the $T$-th graph between domains, and $\mathcal{W}_T$ would be large when the distributions of the graphs between domains show large discrepancy.
% By assigning larger weights to the graphs with larger distribution discrepancies between domains, we prioritize alignment in those graphs. This adaptive weighting scheme allows us to better adapt the model to the evolving distributions between domains. Furthermore, we also introduce two hyperparameters $\lambda_{SCA}$ and $\lambda_{SCA}$ to balance the effect of iSFA and iSCA respectively.



% \paragraph{Exo-feature alignment.}
% % \noindent
% % \textbf{Exo-feature alignment}: 
% To reduce the domain discrepancy at the global level, we enforce restrictions on the global features mapped by sensor features between domains. Specifically, we first learn global features from sensor features in sequential graphs, where we stack the sensor features in each graph and then stack the features of all graphs. Subsequently, a MLP network is employed to map the stacked features, resulting in the global features $\mathcal{P}^s$ and $\mathcal{P}^t$ in source and target domains, as shown in Fig. \ref{fig:corralign} \textbf{Right}.
% With these global features, we can then align them with Deep Coral, expressed as $\mathcal{L}=\mathcal{M}_c(\mathcal{P}^s,\mathcal{P}^t)$.
% as shown in the exo-feature alignment of Eq. (\ref{eq:exo}).
% As shown in Fig. \ref{fig:corralign} \textbf{Right}, we stack the sensor features in each graph and and map the stacked features to the global features, which are then aligned by Deep Coral \cite{10.1007/978-3-319-49409-8_35}. The exo-feature alignment can be shown as Eq. (\ref{eq:exo}).:
% Meanwhile, we adopt deep coral \cite{10.1007/978-3-319-49409-8_35} to make the exo-feature alignment as Eq. (\ref{eq:exo}).
% \begin{equation}
%     \label{eq:exo}
%     \begin{split}
%         h^s = f_{exo}(p_1^s,...,p_N^s) &= \sigma(cat(p_1^s,...,p_N^s)W_{exo})\in\mathbb{R}^{F},\\
%         h^t = f_{exo}(p_1^t,...,p_N^t) &= \sigma(cat(p_1^t,...,p_N^t)W_{exo})\in\mathbb{R}^{F},\\
%         C^s &= \frac{(h^s)^Th^s - \frac{1}{B^s}(1^Th^s)(1^Th^s)}{B^s-1},\\
%         C^t &= \frac{(h^t)^Th^t - \frac{1}{B^t}(1^Th^t)(1^Th^t)}{B^t-1},\\
%         \mathcal{L}_{EXO} &= \frac{1}{4F^2}||C^s-C^t||_F^2,
%     \end{split}
% \end{equation}
% where $cat(\cdot)$ represents concatenation. $||\cdot||_F^2$ is the squared matrix Frobenius norm. $B^s$ and $B^t$ are the number of samples in the source and target domains. 
% Finally, the overall loss function (\ref{eq:overloss}) is minimized:
% \begin{equation}
%     \label{eq:overloss}
%     \begin{split}
%         \mathcal{L} &= \mathcal{L}_C + \mathcal{L}_{EXO} + \mathcal{L}_{Endo},
%     \end{split}
% \end{equation}
% where $\mathcal{L}_C$ is the cost function (i.e., Mean Square Error loss or Cross Entropy loss, depending on the specific tasks) computed by the source data and labels.

